A two-scale computational homogenization approach for elastoplastic truss-based lattice structures

The revolutionary advancements in metal additive manufacturing have enabled the production of alloy-based lattice structures with complex geometrical features and high resolutions. This has encouraged the development of nonlinear material models, including plasticity, damage, etc., for such materials. However, the prohibitive computational cost arising from the high number of degrees of freedom for engineering structures composed of lattice structures highlights the necessity of homogenization techniques, such as the two-scale computational homogenization method. In the present work, a two-scale homogenization approach with on-the-fly exchange of information is adopted to study the elastoplastic behavior of truss-based lattice structures. The macroscopic homogenized structure is represented by a two-dimensional continuum, while the underlying microscale lattices are modeled as a network of one-dimensional truss elements. This helps to significantly reduce the associated computational cost by reducing the microscopic degrees of freedom. The microscale trusses are assumed to exhibit an elastoplastic material behavior characterized by a combination of nonlinear exponential isotropic hardening and linear kinematic hardening. Through multiple numerical examples, the performance of the adopted homogenization approach is examined by comparing forces and displacements with direct numerical simulations of discrete structures for three types of stretching-dominated lattice topologies, including triangular, X-braced and X-Plus-braced unit cells. Furthermore, the principle of scale separation, which emphasizes the need for an adequate separation between the macroscopic and microscopic characteristic lengths, is investigated.

==> extra.tex <==
% Inserting the definition of $\bm{d}$ from Eq. \ref{eq:8} into Eq. \ref{eq:18}, the final form of the equilibrium equation can be written as

% \begin{equation}
% \label{eq:19}
%     \bm{B}_{0}^{T}\bm{K}_{uc} \left( \bm{B}_{0} \bm{d}_{0} + \bm{B}_{e} \bm{e} \right) = \bm{0}.
% \end{equation}

% By solving Eq. \ref{eq:19}, the primary unknowns of the system of the equations, i.e., DoFs of the independent nodes $\bm{d}_0$, can be obtained in terms of the macroscopic strain field $\bm{e}$. The existence and uniqueness of the obtained solutions was shown in \cite{vigliotti2012linear}. 


% \begin{equation}
% \label{eq:20}
%     \bm{R}^i = \bm{B}_{0}^{T}\bm{f}^{i}
% \end{equation}

% \begin{equation}
% \label{eq:21}
%     \bm{d}_{0}^{i+1} = \bm{d}_{0}^{i} - \left( \left. \dfrac{\partial{\bm{R}}}{\partial{\bm{d}_{0}}} \right|^{i} \right)^{-1} \bm{R}^{i}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \dfrac{\partial{\bm{R}}}{\partial{\bm{d}_{0}}} = \dfrac{\partial{\bm{R}}}{\partial{\bm{f}}} \; \dfrac{\partial{\bm{f}}}{\partial{\bm{d}}} \; \dfrac{\partial{\bm{d}}}{\partial{\bm{d}_{0}}} = \bm{B}_{0}^{T} \, \dfrac{\partial{\bm{f}}}{\partial{\bm{d}}} \, \bm{B}_{0}
% \end{equation}


% \begin{equation}
% \label{eq:}
%     q = H \varepsilon^{pl}
% \end{equation}


% \begin{equation}
% \label{eq:}
%     \mathbb{E}_{\sigma} = \{  \left( \sigma, q, \alpha \right) \in \mathbb{R} \times \mathbb{R}_+ \times \mathbb{R} \; | \; \Phi(\sigma, q, \alpha) \leq 0 \}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \dot{\lambda} \dot{\Phi}(\sigma, q, \alpha) = 0 \qquad \left( \mathrm{if} \; \Phi(\sigma, q, \alpha) = 0 \right)
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \sgn{(\sigma-q)} E \left( \dot{\varepsilon} - \dot{\varepsilon}^{pl} \right) - sgn{(\sigma-q)} H \dot{\varepsilon}^{pl} - Q_{\infty} b \, \mathrm{e}^{- b \alpha} \dot{\alpha} = 0
% \end{equation}

% \begin{equation}
% \label{eq:}
%      \sgn{(\sigma-q)} E \dot{\varepsilon} -  E \dot{\lambda} - H \dot{\lambda} - Q_{\infty} b \, \mathrm{e}^{- b \alpha} \dot{\lambda} = 0
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \sigma_{n+1} = \sigma_{n+1}^{trial} - E \Delta\lambda \sgn{ \left( \sigma_{n+1} - q_{n+1} \right)}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \sigma_{n+1} - q_{n+1} = \sigma_{n+1}^{trial} - q_{n}- \left( E + H \right) \Delta\lambda \sgn{ \left( \sigma_{n+1} - q_{n+1} \right)}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \Phi_{n+1} = \left| \sigma_{n+1} - q_{n+1} \right| - \sigma_{y} \left( \alpha_{n+1} \right) = 0
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \sigma_{n+1} = \sigma_{n+1}^{trial} - E \Delta \lambda \sgn{ \left( \sigma_{n+1}^{trial} - q_{n} \right)}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \varepsilon_{n+1}^{pl} = \varepsilon_{n}^{pl} + \Delta \lambda \sgn{ \left( \sigma_{n+1}^{trial} - q_{n} \right)}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     q_{n+1} = q_{n} + H \Delta \lambda \sgn{ \left( \sigma_{n+1}^{trial} - q_{n} \right)}
% \end{equation}

% \begin{equation}
% \label{eq:}
%     \alpha_{n+1} = \alpha_{n} + \Delta \lambda
% \end{equation}


% \begin{table}[]
% \label{tab:}
% \caption{Caption}
% \centering
%     \begin{tabular}{p{\linewidth}}
%     \toprule
%     $R = f_{n+1}^{trial} - \left( E + H \right) \Delta \lambda - \sigma_{y} \left( \alpha_{n+1} \right) + \sigma_{y} \left( \alpha_{n} \right)$\\
%     $\dfrac{\mathrm{d} R}{\mathrm{d} \Delta \lambda} = - \left( E + H \right) - Q_{\infty} b \, \mathrm{e}^{-b \left( \alpha_{n} + \Delta \lambda \right)}$ \\
%     \bottomrule
%     \end{tabular}
% \end{table}

% and fine resolutions (i.e., a substantial surge in the quantity of individual struts)

% Employing FEM, the array of nodal forces $\bm{f}$ is determined by 

% \begin{equation}
% \label{eq:17}
%     \bm{f} = \bm{K}_{uc} \bm{d},
% \end{equation}
